DAM: Towards A Foundation Model for Time Series Forecasting

It is challenging to scale time series forecasting models such that they forecast accurately for multiple distinct domains and datasets, all with potentially different underlying collection procedures (e.g., sample resolution), patterns (e.g., periodicity), and prediction requirements (e.g., reconstruction vs. forecasting). We call this general task universal forecasting. Existing methods usually assume that input data is regularly sampled, and they forecast to pre-determined horizons, resulting in failure to generalise outside of the scope of their training. We propose the DAM - a neural model that takes randomly sampled histories and outputs an adjustable basis composition as a continuous function of time for forecasting to non-fixed horizons. It involves three key components: (1) a flexible approach for using randomly sampled histories from a long-tail distribution, that enables an efficient global perspective of the underlying temporal dynamics while retaining focus on the recent history; (2) a transformer backbone that is trained on these actively sampled histories to produce, as representational output, (3) the basis coefficients of a continuous function of time. We show that a single univariate DAM, trained on 25 time series datasets, either outperformed or closely matched existing SoTA models at multivariate long-term forecasting across 18 datasets, including 8 held-out for zero-shot transfer, even though these models were trained to specialise for each dataset-horizon combination. This single DAM excels at zero-shot transfer and very-long-term forecasting, performs well at imputation, is interpretable via basis function composition and attention, can be tuned for different inference-cost requirements, is robust to missing and irregularly sampled data {by design}.

==> 01_intro.tex <==


Forecasting time-series data is widely used in many domains including weather, traffic, electricity, finance, and cloud resource management.  One challenge with time-series forecasting is the lack of a universal forecasting model (more broadly known as a \textbf{foundation model}) that is applicable to \emph{any} dataset without constraints on its specific properties. Universal time series forecasting is the \emph{general} problem of predicting future values of time-dependent variables from past observations, while making no assumptions that limit the generating mechanism behind the variables~\cite{}.

Building and training  a `universal forecaster' requires the following. The model must (1) be invariant to the specific properties of time series datasets (e.g., continuity, resolution, multi-periodicity, stationarity), and (2) maintain flexibility regarding the forecast it produces (e.g., via a non-fixed forecast horizon). According to this definition, multiple, independently trained, \textbf{variants} of a single design are not a universal forecaster because each variant will be configured (and trained) on a specific combination of datasets, data properties, and forecast horizon. A universal forecaster must be simultaneously \emph{trainable} on a variety of data sources in order to leverage the advantages gained by big data. 

% Given the challenges associated with universal forecasting, why even pursue this paradigm? 
% Due to their importance, techniques for computing a universal representation of time series data has been sought for decades \citep{vovk1992universal, hu2023contrastive, zhang2022self, han2023capacity}; 

The rise of foundation models in other fields (e.g., natural language and computer vision)~\citep{bommasani2021opportunities} suggests that a universal forecaster should be pursued. Aside from the potential performance gains, deploying a universal forecaster is simple compared to training many variants of a single design and deploying them per use-case. To this end, the pursuit of universal forecasting has been ongoing for decades \citep{vovk1992universal, hu2023contrastive, zhang2022self, han2023capacity}. A number of recent advances \citep{nie2022time, wu2022timesnet, kim2021reversible} have taken steps toward universal forecasting by way of training on multiple datasets and remedying distribution shift concerns. Recent state-of-the-art (SoTA) methods \citep{das2023long, nie2022time} evidence what is possible using well-justified model design and training regimes

% For example, consider that deploying a forecasting model in the cloud resource domain often invokes a change in the data distribution (e.g., the scheduling algorithm makes different choices, thus changing the data over time): an overly rigid model (trained on a single dataset) will be subject to performance degradation owing to distribution shift (TODO CITE NON STATIONARY AND INV).


Despite recent advances, even modern methods remain overly rigid regarding input data properties and forecast horizons, meaning that their potential as universal forecasters is limited. Rigid model design is a direct consequence of the heterogeneous nature of time series datasets. Diverse dataset characteristics, such as sample resolution, and use-case requirements, have resulted in constraints that tend to govern model design; for simplicity, we group constraints into two categories:
\begin{enumerate}
    \item \textbf{Context constraints}: existing methods typically expect context data as a fixed-length sequence with regular intervals [TODO CITE IRREGULAR]. Single dataset and single resolution training is a long-standing practice in the forecasting domain. This, in turn, forces short training times CITE TODO that mitigate overfitting in the small data regime. 
    % It is challenging to apply existing models to universal forecasting because of the design principles followed to create them.
    \item \textbf{Forecast constraints}: the current norm is to forecast directly over a fixed-length horizon by designing a model to produce a vector (per variable) over the horizon. Models are then optimised to target specific horizons and a single dataset in order to maximise performance. In most cases this design choice disables task transfer (e.g., imputation using a forecasting model) or very long-term forecasting (beyond the fixed horizon) without either different training runs/setups or autoregressive methods, respectively. 
\end{enumerate}

% \textbf{fixed-length sequential data as inputs} and \textbf{fixed forecast horizons}. 

\paragraph{Discarding constraints}
In this paper we present the deep data-dependant approximate analytical model (D\textsuperscript{3}A\textsuperscript{2}M, or DAM for simplicity) as a foundational model for universal forecasting. The DAM is not subject to context or forecast constraints by design. The DAM is a transformer that consumes non-sequential \textbf{historically sampled} time-value pairs (see Section \ref{sec:DAM-time}) to produce a continuous approximate analytical \textbf{time-dependant function as output} (see Section \ref{sec:DAM-basis}). This function is composed of a small set of sinusoidal basis functions. We show in this paper that such a constrained functional space, adjusted by a powerful backbone model, is sufficient for SoTA forecasting and imputation (see Sections \ref{sec:experiments} and \ref{sec:experiment-imputation}). 

% Intuitively, the DAM replaces humans in the `classical' forecasting regime, where individual models are applied for trends, seasonalities, and residual components TODO CITE PROPHET. Strictly speaking, the DAM produces as a representation the parameters\footnote{Note that these parameters are \textbf{not weights} within the model, but the output itself} of many continuous basis functions that can be assessed at some query time. 



% \textbf{Lifting the context constraints} requires a model that is not reliant on or limited by the properties of individual datasets or variables therein. Such a model can be applied to any time series without concern for resolution differences, context length, inconsistent data collection or missing data. \textbf{Lifting forecast constraints} requires a model that is not limited to producing forecasts over a pre-selected horizon. We acknowledge that it is possible to edit datasets (e.g., using imputation and up/down-scaling) such that they can be ingested by existing models, and that autoregressive techniques effectively mitigate fixed horizons, but these techniques are symptomatic treatments of the underlying problems with existing methods: they are not designed to solve the \textbf{general forecasting task}, but rather to forecast sufficiently well for a highly constrained setup. This does not mean that existing methods are without merit, but rather that long-standing practices in time series forecasting need reconsideration.


% Training models to solve the general forecasting task is challenging owing to some inherent characteristics of time series data. Time series datasets: (1) are usually smaller (i.e.,~shorter \citep{li2022generative}) than datasets from other domains, (2) consist of observations that are typically dependent on other observations (i.e., violates i.i.d.~assumptions), and (3) can have different generating mechanisms that produce incompatible properties (such as resolution and continuity). 


% Most existing state-of-the-art methods make two important simplifying assumptions about the forecasting task. First, time series data is sequential. Second, forecasts should occur over fixed horizons. We argue in this paper that these assumptions limit model design such that building a universal forecaster is out of reach. A model that leverages sequentiality (TODO CITE) is limited to fixed resolution inputs and a maximum history of exactly the length of the input sequence. 

% It is often suggested that the sequential nature of time series enables better performance are optimised on a single dataset because of these incompatible properties across datasets, and therefore practitioners must rely on heuristic mechanisms to avoid overfitting (e.g., early stopping). [TODO CITE] showed how simple linear models often outperform complex methods, further evidencing how overfitting is a major challenge in forecasting. We propose that the general task of ``predicting the future given the past'' is not sufficiently represented by a single small dataset or source. To solve this general task we require a \textbf{universal forecaster} that can be trained across a large number of time series datasets.

% \subsection{Rethinking forecasting}
% One `classical' approach to forecasting is to construct a forecast additively by first modelling the long-term trend (e.g., via polynomials), next the periodic elements (e.g., via FFT extrapolation), and thereafter the residual components (e.g., via ARIMA [TODOCITE] or a small MLP). Applying use-case-specific models to these components, based on data analysis and cost constraints, is common practice and still widely accepted despite the potential performance advantages of deep SoTA approaches. Modern methods often involve complexities -- methodological, during training, and for deployment -- that discourage real-world practitioners from adopting such methods. The fact that all current SoTA methods (to our best knowledge) must be trained with fixed-length input and output sequences is an additional discouragement. 

% \paragraph{Discarding sequentiality and forecast horizons}
% We designed the DAM to be unconstrained regarding context and forecast horizons, while also being \textbf{cost-flexible during inference}. We discarded sequentiality and forecast horizons in favour of generality and flexibility to design the deep data-dependent approximate analytical model (DAM) for universal forecasting. The DAM is a transformer that consumes non-sequential \textbf{historically sampled} time-value pairs, thus mitigating differences in dataset properties and enabling new and intuitive mechanisms for history ingestion (see Section TODO). The representation the DAM produces is then interpreted as the parameters of an analytical function of time\footnote{Note that these parameters are \textbf{not weights} within the model, but rather the output it produces after processing input data}. This interpretation enables forecast flexibility because such a function can be assessed cheaply (compared to a forward pass through a neural network) for any query time (back or forward). 

To our best knowledge the DAM is the first time series foundation model to be trained on a large collection of publicly available time series datasets to achieve SoTA on TODO. Specifically, the DAM was trained on 10 benchmark datasets, totaling 1290 variables and over 22 million data points, effectively mitigating the overfitting issues often found in the time series (TODO: CITE 5 EPOCHS). Every experiment in the main body of this paper was conducted \textbf{using a single univariate DAM, without fine-tuning}. In the remainder of this paper we present the DAM in more detail and explore the benefits and insights now available as a consequence of targeting universal forecasting by \textbf{DAMing}. These benefits constitute our contributions:

% , but with a post-hoc-trained `multivariator' mixing model to leverage cross-variable dependencies. 

% The DAM also produces interpretable forecasts because (1) input flexibility enables sample uncertainty as a tool for understanding the impact of specific data on a forecast (see Section TODO), and (2) the analytical function over time is composed as a sum of basis functions, meaning lower frequency components can be analysed for long-term trends (for example).

% \paragraph{The DAM is a big model, trained on big data, to forecast as humans often do.} In some sense the DAM uses a powerful transformer architecture to accomplish the task humans have been undertaking for years in the classical forecasting regime. It looks at the past data to produce a large set of parameterised basis functions that are not unlike the trend, seasonal, and residual decomposition approach followed by practitioners -- one of the most widely used trusted forecasting models is based on Facebook Prophet TODO:CITE and uses such a multi-part approach. The DAM learns how to generalise this process because it is trained on many datasets that have diverse properties and patterns.

% We trained \textbf{a single univariate DAM} on TODO:13 benchmark data sources, totally 1490 unique univariate variables and over 31 million data points. The DAM yielded state-of-the-art performance across TODO:RESULTS. 

\begin{enumerate}
\item The DAM for universal forecasting, a foundational model for time series tasks, evidincing SoTA forecasting performance on TODO. 
\item A history sampling regime that enables efficient access to the distant past and reflects an intuitive approach to temporal information.
\item A fully differentiable output representation interpreted as the weights of basis functions, enabling prediction at any time with a single forward pass.
\item Demonstrations of the DAM's flexibility, tunable inference cost, ability to forecast very long-term, transfer to unseen tasks/datasets, and interpretability.
% and the use of multi-scale basis functions as the analytical function.
\end{enumerate}

This remainder paper is structured as follows. In Section \ref{sec:method} we detail the DAM, how it uses a new treatment of time by way of a historical sampling regime, and how basis functions are the mechanism for prediction. In Section \ref{sec:experiments} we present experiments on forecasting, transfer to unseen datasets and an unseen task. In Section \ref{sec:demo} we demonstrate and analyse the DAM's utility regarding flexible inference cost, basis function compositions, attention analysis for interpretability, and various ablations.

% This paper is structured to demonstrate challenges in long-term forecasting and provide evidence of the superiority of the DAM when facing these challenges. Where possible we provide direct comparisons against a set of competitors models that represent the previous state-of-the-art in forecasting (to our best knowledge and as of the time of writing). We begin in Section TODO by detailing the DAM architecture and show how we designed it to ingest non-sequential time series and generate an approximate analytical function of time. In Section TODO we expound upon the challenges that inspired us to create the DAM. We give standard long-term forecasting results in Section TODO.1 as the first point of call for readers who are familiar with existing forecasting work.

% Consequently, model overfitting is widespread and difficult to overcome. More importantly, 

% Univariate, multivariate, and global univariate forecasting paradigms represent the majority of historical approaches. Unfortunately, time series datasets are typically 

% The global univariate forecasting paradigm involves applying a single model/predictor to multiple, often related, univariate time series. In some sense, global forecasters aim to solve the more general task of `predict the future given the past', whereas univariate forecasters are constrained to solve this task for a single variable only. Earlier research [TODO CITE] has shown that global forecasters perform similarly to univariate forecasters. Multivariate forecasters are also applicable to multiple variables, but are constrained to the set of variables on which they are trained. All three of the aforementioned paradigms are almost always constrained by assumptions on the generating mechanism behind the variables (e.g., resolution).

% The universal forecasting paradigm is the natural extension of global forecasting, with the primary difference being the lifting of assumptions on the underlying variables' generating mechanisms. A universal forecaster should be applicable to many multiple variables from diverse sources, ingest data of various lengths, resolutions, and with variable trend and periodicity scales, handle seamlessly missing data, and forecast over multiple horizons and at multiple resolutions. 

% Designing and training a model that is able to serve the universal forecasting paradigm is extremely challenging as it requires rethinking the typical assumptions made when designing forecasting models. First, lifting restrictions on input data continuity and resolution necessitated a transformer architecture for data ingestion, and consequently enabled highly flexible inputs. Second, requiring forecasts at multiple resolutions and forecast horizons necessitated a basis function approach to prediction, where forecasts are made by evaluating an analytical function at a given time. The DAM combines a powerful modern neural network architecture to predict the parameters of a set of basis functions over time. 

% Importantly, the basis function parameters at any given time (for a given variable) are the \textbf{output} of the DAM, meaning that they constitute what is typically considered the `predictions'. Intuitively, the DAM attempts to build a solution much like a human would build a `classical' solution: analyse the target dataset, choose and combine multiple forecasts (e.g., a polynomial for long term trends, a FFT for periodicity, and a residual model for fine-grained adjustment). 

% In this paper we detail The DAM for universal forecasting (in Section TODO), show how it outperformers many existing univariate and multivariate forecasters, demonstrate its flexibility, applicability, and interpretability. Our contributions are:

